DDIPrompt: Drug-Drug Interaction Event Prediction based on Graph Prompt Learning

Drug combinations can cause adverse drug-drug interactions(DDIs). Identifying specific effects is crucial for developing safer therapies. Previous works on DDI event prediction have typically been limited to using labels of specific events as supervision, which renders them insufficient to address two significant challenges: (1) the bias caused by \textbf{highly imbalanced event distribution} where certain interaction types are vastly under-represented. (2) the \textbf{scarcity of labeled data for rare events}, a pervasive issue where rare yet potentially critical interactions are often overlooked or under-explored due to limited available data. In response, we offer ``DDIPrompt'', an innovative solution inspired by the recent advancements in graph prompt learning. Our framework aims to address these issues by leveraging the intrinsic knowledge from pre-trained models, which can be efficiently deployed with minimal downstream data. Specifically, to solve the first challenge, DDIPrompt features a hierarchical pre-training strategy to foster a generalized and comprehensive understanding of drug properties. It captures intra-molecular structures through augmented links based on structural proximity between drugs, further learns inter-molecular interactions emphasizing edge connections rather than concrete catagories. For the second challenge, we implement a prototype-enhanced prompting mechanism during inference. This mechanism, refined by few-shot examples from each category, effectively harnesses the rich pre-training knowledge to enhance prediction accuracy, particularly for these rare but crucial interactions. Extensive experiments on two benchmark datasets demonstrate DDIPrompt's SOTA performance, especially for those rare DDI events.

==> archive_old_content.tex <==
%%%% Old Abs 

  Predicting drug-drug interaction adverse events, so-called DDI events, is increasingly valuable as it facilitates the study of mechanisms underlying drug use or adverse reactions. Existing models often neglect the distinctive characteristics of individual event classes when integrating multi-source features, which contributes to systematic unfairness when dealing with highly imbalanced event samples. Moreover, the limited capacity of these models to abstract the unique attributes of each event subclass considerably hampers their application in predicting rare drug-drug interaction events with a limited sample size. Reducing dataset bias and abstracting event subclass characteristics are two unresolved challenges. Recently, prompt tuning with frozen pre-trained graph models, namely "pre-train, prompt, fine-tune" strategy, has demonstrated impressive performance in few-shot tasks. Motivated by this, we propose DDIPrompt as a solution to address these aforementioned challenges. Specifically, our proposed approach entails a hierarchical pre-training task that aims to capture crucial aspects of drug molecular structure and intermolecular interactions while effectively mitigating implicit dataset bias within the node embeddings. Furthermore, we construct a prototypical graph by strategically sampling data from distinct event types and design subgraph prompts utilizing pre-trained node features. Through comprehensive benchmark experiments, we validate the efficacy of our subgraph prompts in accurately representing event classes and achieve exemplary results in both overall and subclass prediction tasks.


\section{Experiment}
% 有一些细节，比如GraphSAGE因为我在method里写过，我就省过去了。
% 把内容拆成了 【实现细节】 和 【验证指标】两部分
% To verify the effectiveness of DDIPrompt on the few-sample data set, we randomly sampled 20\% of the samples in each event class as the training set, the rest for test. We implement all the baselines and our method with PyTorch. Since predicting DDI events is a multi-class classification task, we adopt several evaluation metrics, including Accuracy, Macro-F1, Macro-Recall and Macro-Precision under a multi-class setting. In the hierarchical pre-training stage, for molecule similarity score prediction, we respectively select K=10 nodes that are most similar and least similar to each drug to form the final drug neighbor graph. For link prediction, a two-layer GraphSage Convolutional layer and an MLP classification head are employed, with a maximum epoch of 1000. In prompt-tuning stage, we use Adam \cite{adam} optimizer with the learning rate of 0.002. The dropout starts at 0.3 and increases by 0.05 per training round until reaching a maximum rate of 0.9. After reaching the maximum rate, it remains constant during training. A two-layer MLP classification head with a maximum epoch of 300 was employed for DDI event prediction, and the best performing models based on the Accuracy and Macro-F1 on the test set. For rare events group, We record the mean and variance of the five results as the final experimental results. More details on our hyperparameter search procedure are given in Appendix.


% Table on Deng's dataset with STD

  % \multirow{4}{*}{Rare     } & Acc & 0.3636$\pm$0.0228 & 0.4117$\pm$0.0088 & 0.4597$\pm$0.0005 & 0.4727$\pm$0.0026 & \underline{0.5513$\pm$0.0285} & 0.5216$\pm$0.0172 & \textbf{0.6494$\pm$0.0006} & 17.79 \\
        %                            & F1  & 0.3186$\pm$0.0084 & 0.3804$\pm$0.0105 & 0.4438$\pm$0.0025 & 0.4375$\pm$0.0018 & \underline{0.5101$\pm$0.0145} & 0.4834$\pm$0.0016 & \textbf{0.6360$\pm$0.0015} & 24.69 \\
        %                            & Rec & 0.3062$\pm$0.0006 & 0.3721$\pm$0.0078 & 0.4321$\pm$0.0015 & 0.4373$\pm$0.0002 & \underline{0.4828$\pm$0.0076} & 0.4817$\pm$0.0008 & \textbf{0.6508$\pm$0.0008} & 34.80 \\
        %                            & Pre & 0.3412$\pm$0.0184 & 0.3972$\pm$0.0125 & 0.4507$\pm$0.0030 & 0.5696$\pm$0.0123 & \underline{0.5957$\pm$0.0258} & 0.4938$\pm$0.0024 & \textbf{0.7220$\pm$0.0018} & 21.20 \\

% Table on Ryu's with STD

 % \multirow{4}{*}{Rare     } & Acc & 0.4243$\pm$0.0125 & 0.5617$\pm$0.0082 & 0.6428$\pm$0.0064 & 0.6667$\pm$0.0137 & \underline{0.6958$\pm$0.0135} & 0.6238$\pm$0.0016 & \textbf{0.8847$\pm$0.0007} & 27.15 \\
        %                            & F1  & 0.3723$\pm$0.0075 & 0.5237$\pm$0.0036 & 0.5978$\pm$0.0016 & 0.6121$\pm$0.0048 & \underline{0.6421$\pm$0.0086} & 0.5823$\pm$0.0007 & \textbf{0.8676$\pm$0.0009} & 35.12 \\
        %                            & Rec & 0.3444$\pm$0.0008 & 0.5014$\pm$0.0015 & 0.5718$\pm$0.0008 & 0.5816$\pm$0.0035 & \underline{0.6037$\pm$0.0115} & 0.5590$\pm$0.0005 & \textbf{0.8661$\pm$0.0011} & 43.47 \\
        %                            & Pre & 0.4409$\pm$0.0215 & 0.5319$\pm$0.0075 & 0.6636$\pm$0.0082 & 0.6617$\pm$0.0105 & \underline{0.6558$\pm$0.0205} & 0.5932$\pm$0.0008 & \textbf{0.9013$\pm$0.0003} & 37.44 \\



\begin{table*}[!t]

   \small
   \centering

    \caption{\textbf{Overall Performance on Deng's Dataset}. The best and second-best results are highlighted with \textbf{bold} and \underline{underline}, respectively.}
    \label{exp:deng_overall}
   % \resizebox{\textwidth}{!}{%
    
    \begin{tabular}{cc|cccccc|cc}
       \toprule
        &  &  DeepDDI & SSI-DDI & MUFFIN & MRCGNN & META-DDIE & D2PT & DDIPrompt & Improv \% \\
      \midrule
        
       \multirow{4}{*}{All Events} & Acc & 0.5794 & 0.6829 & 0.7458 & \underline{0.7701} & 0.7329 & 0.6413 & \textbf{0.7858} & 2.04 \\
                                   & F1  & 0.3231 & 0.4037 & \underline{0.4561} & 0.4464 & 0.4148 & 0.3179 & \textbf{0.4874} & 6.86 \\
                                   & Rec & 0.2835 & 0.3949 & \underline{0.4418} & 0.4307 & 0.3812 & 0.2801 & \textbf{0.4533} & 2.60 \\
                                   & Pre & 0.3318 & 0.4538 & 0.4789 & \underline{0.4808} & 0.4582 & 0.3521 & \textbf{0.5765} & 19.90 \\
       \midrule

       \multirow{4}{*}{Common    } & Acc & 0.5915 & 0.6760 & 0.7571 & \underline{0.7823} & 0.7560 &  0.6621 & \textbf{0.8041} & 2.79 \\
                                   & F1  & 0.3426 & 0.4806 & 0.5580 & \underline{0.5824} & 0.5524 & 0.3286 & \textbf{0.6403} & 9.94 \\
                                   & Rec & 0.3167 & 0.4792 & 0.5361 & \underline{0.5476} & 0.5412 & 0.3221 & \textbf{0.6199} & 13.20 \\
                                   & Pre & 0.3735 & 0.4998 & 0.6083 & \underline{0.6587} & 0.5917 & 0.3498 & \textbf{0.6917} & 5.01 \\
       \midrule

       \multirow{4}{*}{Fewer     } & Acc & 0.4718 & 0.6440 & 0.7340 & \underline{0.8189} & 0.7685 & 0.7300 & \textbf{0.8862} & 8.22 \\
                                   & F1  & 0.4191 & 0.6173 & 0.7201 & \underline{0.7992} & 0.7412 & 0.6832 & \textbf{0.8758} & 9.58 \\
                                   & Rec & 0.4119 & 0.6008 & 0.7002 & \underline{0.7779} & 0.7257 & 0.6778 & \textbf{0.8735} & 12.29 \\
                                   & Pre & 0.4544 & 0.6421 & 0.7381 & \underline{0.8036} & 0.7543 & 0.7021 & \textbf{0.8831} & 9.89 \\
        \midrule

        \multirow{4}{*}{Rare}   & Acc & 0.3636 & 0.4117 & 0.4597 & 0.4727 & \underline{0.5513} & 0.5216 & \textbf{0.6494} & 17.79 \\ 

        & F1 & 0.3186 & 0.3804 & 0.4438 & 0.4375 & \underline{0.5101} & 0.4834 & \textbf{0.6360} & 24.69 \\ 

        & Rec & 0.3062 & 0.3721 & 0.4321 & 0.4373 & \underline{0.4828} & 0.4817 & \textbf{0.6508} & 34.80 \\ 

        & Pre & 0.3412 & 0.3972 & 0.4507 & 0.5696 & \underline{0.5957} & 0.4938 & \textbf{0.7220} & 21.20 \\
       \bottomrule
    \end{tabular}%
    % }
\end{table*}


\begin{table*}[!t]
   \small
   \centering
    \caption{\textbf{Overall Performance on Ryu's Dataset}. The best and second-best results are highlighted with \textbf{bold} and \underline{underline}, respectively.}
    \label{exp:ryu_overall}
    
    %\resizebox{\textwidth}{!}{%
    \begin{tabular}{cc|cccccc|cc}
       \toprule
        &  &  DeepDDI & SSI-DDI & MUFFIN & MRCGNN & META-DDIE & D2PT & DDIPrompt & Improv \% \\
      \midrule
        
       \multirow{4}{*}{All Events} & Acc & 0.7518 & 0.7658 & 0.8532 & \underline{0.8754} & 0.8030 & 0.7552 & \textbf{0.8964} & 2.40 \\
                                   & F1  & 0.5457 & 0.5121 & 0.6541 & \underline{0.7411} & 0.6126 & 0.5349 & \textbf{0.7489} & 1.05 \\
                                   & Rec & 0.5178 & 0.5002 & 0.6225 & \underline{0.7104} & 0.5930 & 0.5217 & \textbf{0.7146} & 0.59 \\
                                   & Pre & 0.5951 & 0.5478 & 0.6995 & \underline{0.7654} & 0.6437 & 0.5586 & \textbf{0.8291} & 8.32 \\
       \midrule

       \multirow{4}{*}{Common    } & Acc & 0.7764 & 0.7775 & 0.8573 & \underline{0.8862} & 0.8419 & 0.7593 & \textbf{0.8912} & 0.56 \\
                                   & F1  & 0.5518 & 0.5333 & 0.6657 & \underline{0.7341} & 0.6612 & 0.5239 & \textbf{0.7937} & 8.12 \\
                                   & Rec & 0.5336 & 0.5201 & 0.6354 & \underline{0.7261} & 0.6311 & 0.5178 & \textbf{0.7718} & 6.29 \\
                                   & Pre & 0.6001 & 0.5512 & 0.7495 & \underline{0.7509} & 0.6768 & 0.5563 & \textbf{0.8654} & 15.25 \\
       \midrule

       \multirow{4}{*}{Fewer     } & Acc & 0.6517 & 0.7221 & 0.8312 & \underline{0.9016} & 0.8406 & 0.7860 & \textbf{0.9628} & 6.79 \\
                                   & F1  & 0.6232 & 0.7115 & 0.7856 & \underline{0.8906} & 0.7925 & 0.7414 & \textbf{0.9575} & 7.51 \\
                                   & Rec & 0.6061 & 0.7003 & 0.7593 & \underline{0.8894} & 0.7743 & 0.7301 & \textbf{0.9579} & 7.70 \\
                                   & Pre & 0.6413 & 0.7226 & 0.8092 & \underline{0.8911} & 0.8147 & 0.7817 & \textbf{0.9616} & 7.91 \\
        \midrule



        \multirow{4}{*}{Rare} & Acc & 0.4243 & 0.5617 & 0.6428 & 0.6667 & \underline{0.6958} & 0.6238 & \textbf{0.8847} & 27.15 \\ 

        & F1 & 0.3723 & 0.5237 & 0.5978 & 0.6121 & \underline{0.6421} & 0.5823 & \textbf{0.8676} & 35.12 \\

        & Rec & 0.3444 & 0.5014 & 0.5718 & 0.5816 & \underline{0.6037} & 0.5590 & \textbf{0.8661} & 43.47 \\ 

        & Pre & 0.4409 & 0.5319 & \underline{0.6636} & 0.6617 & 0.6558 & 0.5932 & \textbf{0.9013} & 37.44 \\ 
         
       \bottomrule
    \end{tabular}%
    %}
\end{table*}


% We summarize the results for both data sets in Tables 2 and 3, where the best results are shown in bold and the suboptimal results are underlined. We can observe that our proposed DDIPrompt consistently outperforms other baselines for both two datasets, with a significant margin. It is also notable that most of the baselines are not effective when being trained with only few samples, the reasons can be summarized as follows: 1) The performance of DeepDDI, SSI-DDI, and MUFFIN, which primarily rely on analyzing drug molecular structures and DDI event supervision labels, is expected to be unsatisfactory on small samples, particularly when dealing with a limited number of events. DeepDDI, in particular, experiences a significant decline in classification effectiveness under such circumstances, largely due to its struggles in extracting node features for modeling and heavy reliance on supervised samples for training. 2) MRCGNN, META-DDIE, and D2PT have all incorporated strategies to address the challenges posed by small sample problems. META-DDIE utilizes the similarity between pairs of drug molecules to determine the likelihood of shared DDI events. However, the simplicity of the model limits its ability to extract comprehensive features from drug pairs. D2PT, on the other hand, focuses on leveraging weak information in Graph Neural Networks (GNNs) and falls short in adequately capturing the unique characteristics of individual drugs. In the case of MRCGNN, the two-stage molecular feature update process also relies heavily on labels and struggles in effectively handling rare events.

